Formalizing Traceability and Derivability in Software Product Lines

In the literature, the definition of product in a Software Product Line (SPL) is based upon the notion of consistency of the constraints, imposed by variability and traceability relations on the elements of the SPL. In this paper, we contend that consistency does not model the natural semantics of the implementability relation between problem and solution spaces correctly. Therefore, we define when a feature can be {\em derived} from a set of components . Using this, we define a product of the SPL by a <specification, architecture> pair, where all the features in the specification are derived from the components in the architecture. This notion of derivability is formulated in a simple yet expressive, abstract model of a productline with traceability relation. We then define a set of SPL analysis problems and show that these problems can be encoded as Quantified Boolean Formulas. Then, QSAT solvers like QUBE can be used to solve the analysis problems. We illustrate the methodology on a small fragment of a realistic productline.

==> proofs.tex <==
\begin{lemma}(Internal Consistency of Traceability)
Consider a canonical SPL. 
Let TCF, the trace consistency formula be defined as $\forall c_1 \dots c_n. \bigwedge_{f \in F}[f\_prov(f) \Rightarrow f \_ req(f)]$. Then, ${\cal T}$ is  internally consistent iff TCF is true.
 \end{lemma}
\begin{proof}
 Let ${\cal T}$ be the traceability relation. Assume ${\cal T}$ is internally consistent. By definition, this means that $\forall f \in F$ ($F$ is a specification in $\overline{\cal F}$) 
and $\forall C \in {\cal C}$, ($C$ is an architecture in $\overline{\cal C}$)
whenever $C \in prov(f)$, 
there is some $C' \in req(f)$ such that $C' \subseteq C$. Let $prov(f)=\{S_1, \dots, S_k\}$ and $req(f)=\{R_1, \dots, R_l\}$. As seen in the definitions above, we have a set of propositions $Prop(S_j)$ and $Prop(R_j)$ associated to each $S_j$ and $R_j$.
%Given that $C' \subseteq C$ for some $C' \in req(f)$, for any $C \in prov(f)$. 
With each $S_j \in prov(f)$, let $R_{i_j} \in req(f)$ be such that $R_{i_j} \subseteq S_j$. 
Let $J=\{j \mid R_j \subseteq S_n$ for some $S_n \in prov(f)\}$.
$R_{i_j} \subseteq S_j \Rightarrow Prop(R_{i_j}) \subseteq Prop(S_j)$.  This means 
$ \bigwedge_{c \in Prop(S_j)} c \Rightarrow   \bigwedge_{c' \in Prop(R_{i_j})} c'$
for all $S_j \in prov(f)$.   Then 
clearly, for all variables $c_1, \dots, c_n$ in $U_C$, 
($\bigvee_{i=1}^k \bigwedge_{c \in Prop(S_i)} c \Rightarrow   \bigvee_{j \in J} \bigwedge_{c' \in Prop(R_j)} c')$, which implies 
$(\bigvee_{i=1}^k \bigwedge_{c \in Prop(S_i)} c \Rightarrow   \bigvee_{h=1}^l \bigwedge_{c' \in Prop(R_h)} c')$. \\
This is nothing but $\forall c_1 \dots c_n$ $[f \_ prov(f) \Rightarrow f \_ req(f)]$ for all $f \in F$.


Conversely, assume that $\forall c_1 \dots c_n$ $[f \_ prov(f) \Rightarrow f \_ req(f)]$.
Let us write $f \_ prov(f)$ as $\bigvee_j S_j$ where $S_j=\bigwedge_{c \in prop(S_j)} c$. Similarly, 
 $f \_ req(f)$ as $\bigvee_h R_h$ where $R_h=\bigwedge_{c' \in prop(R_h)} c'$. 
We prove the result for  canonial SPLs. Given $\bigvee_{S_j \in prov(f)} S_j \Rightarrow \bigvee_{R_h \in req(f)} R_h$ for all $c \in U_C$. 

Assume that there exists some $S \in prov(f)$ such that $R_h \nsubseteq S$ for every $R_h \in req(f)$. Then $\neg(\bigwedge_{c \in prop(S)} c \Rightarrow \bigwedge_{c' \in prop(R_h)} c')$ for every $R_h \in req(f)$.  Consider an assignment ${\cal A}$ to the variables of $U_C$ which makes $\bigwedge_{c \in prop(S)} c$ true, and  which does not satisfy any other $S_i \in prov(f), S_i \neq S$. This is possible since 
$S$ is not a superset of any other $S_i  \in prov(f)$, by canonicity. Then ${\cal A}$ satisfies 
$\bigvee_{S_j \in prov(f)} S_j$ but does not satisfy any of the $R_h$, since
 $\neg(\bigwedge_{c \in prop(S)} c \Rightarrow \bigwedge_{c' \in prop(R_h)} c')$ for every $R_h \in req(f)$. 
This contradicts the assumption that $\bigvee_{S_j \in prov(f)} S_j \Rightarrow \bigvee_{R_h \in req(f)} R_h$. Therefore, there does not exist any $S \in prov(f)$ such that $R_h \nsubseteq S$ for every $R_h \in req(f)$. Thus, 
internal consistency is preserved. 

Note that if the SPL is not canonical, our proof need not hold good. Consider for example, 
$prov(f)=\{\{c,d\}, \{c,d,e\}\}$ and $req(f)=\{\{d,e\}\}$. Then 
$\bigvee_{S_j \in prov(f)} = [(c \wedge d) \vee (c \wedge d \wedge e)] \equiv (c \wedge d \wedge e)$ and 
 $\bigvee_{R_h \in req(f)} = (d \wedge e)$. Here, $\bigvee_{S_j \in prov(f)} \Rightarrow \bigvee_{R_h \in req(f)}$. 
However, $\{d,e\} \nsubseteq \{c,d\}$. Once we make this SPL canonical, we 
get $prov(f)=\{\{c,d\}\}$ and $req(f)=\{\{d,e\}\}$. Then 
clearly, $\neg[\bigvee_{S_j \in prov(f)} \Rightarrow \bigvee_{R_h \in req(f)}]$. 


%$\forall c_1 \dots c_n (\bigvee_j S_j \Rightarrow \bigvee_h R_h)$, then there exists some 
%$i$ such that $\forall c_1 \dots c_n (\bigvee_j S_j \Rightarrow R_i)$. This is equivalent to 
%$\forall c_1 \dots c_n [\bigwedge_{j}(S_j \Rightarrow R_i)]$. Substituting for $S_j, R_i$ we have 
%$\forall c_1 \dots c_n \bigwedge_j[\{\bigwedge_{c \in Prop(S_j)} c   \Rightarrow \bigwedge_{c' \in Prop(R_i)} c'\}]$.
%Since $Prop(S_j), Prop(R_i) \subseteq U_C$, 
% this is equivalent to  $Prop(R_i) \subseteq Prop(S_j)$ for all $S_j \in prov(f)$. This is same as the requirement 
% for internal consistency which says that $\forall C \in prov(f)$ $\exists C' \in req(f)$ such that $C' \subseteq C$.
 \end{proof}

\begin{lemma}(Implements)
 Given a canonical SPL, a set of components $C$, and a feature $f$, $implements(C, f)$ iff $f \_ implements(c'_{1}, \dots, c'_{n}, f)$ where $Prop(C)=(c'_{1}, \dots, c'_n)$.
\end{lemma}
\begin{proof}
 As usual, we assume the SPL is canonical. Assume $implements(C, f)$ holds. Then by definition,  $\exists C_1 \in prov(f)$ and 
$C_2 \in req(f)$, then $C_2 \subseteq C_1 \subseteq C$. To show that $f \_ implements(c'_{1}, \dots, c'_{n}, f)$. Given $Prop(C)=(c'_{1}, \dots, c'_{n})$.  
$f \_ implements(c'_{1}, \dots, c'_{n}, f)$ is defined as 
%$$\forall c_1 \dots c_n [(\bigwedge \limits_{i,j=1}^k [(c_i \Leftrightarrow c_j)] \wedge \bigwedge \limits_{i=1}^k c_i) \Rightarrow formula \_prov(f)]$$
$$\forall c_1 \dots c_n [\bigwedge \limits_{j=1}^n (c'_{j} \Rightarrow c_{j})
  \Rightarrow formula \_prov(f)]$$

 Since $\exists C_1 \in prov(f)$ such that $C_1 \subseteq C$, whenever $Prop(C_1)(i)=1$, we have $Prop(C)(i)=1$. 
 Therefore, whenever there is an assignment of 1 to component variables in atleast one 
 $C_1    \in prov(f)$, $\bigwedge \limits_{c' \in Prop(C_1)} c'$ holds. 
 Then $formula \_prov(f)$ holds. Hence, $f \_ implements(c'_1, \dots, c'_n, f)$ holds.

Conversely, suppose $f \_ implements(c'_{1}, \dots, c'_{n}, f)$ and $Prop(C)=(c'_{1}, \dots, c'_n)$. By definition of \\ 
$f \_ implements(c'_{1}, \dots, c'_{n}, f)$, whenever 
$c'_j  \Rightarrow c_j$, $\bigvee \limits_{C \in prov(f)}\bigwedge \limits_{c \in C} c$ holds. Thus, there exists some $C' \in prov(f)$ such that $\bigwedge \limits_{c \in C'} c$ holds whenever $c'_j  \Rightarrow c_j$ holds. 
Then, for that $C'$, $Prop(C')(i)=1 \Rightarrow Prop(C)(i)=1$. Then $C' \subseteq C$. By Theorem 15, we have 
$implements(C, f)$.
 \end{proof}
\begin{lemma}(Realizes, Covers)
\label{rc}
 Given a set of components $C$ and a set of features $F$, let $Prop(C)=(c'_{1}, \dots, c'_{n})$ and $Prop(F)=(f'_{1}, \dots, f'_{m})$. Then the following statements hold:
\begin{enumerate}
 \item $C$ covers $F$ iff $f \_ covers(c'_{1}, \dots, c'_{n}, f'_{1}, \dots, f'_{m})$
\item $C$ realizes $F$ iff $f \_ realizes(c'_{1}, \dots, c'_{n}, f'_{1}, \dots, f'_{m})$
\end{enumerate}
\end{lemma}
\begin{proof}
Suppose $Prop(C)=(c'_{1}, \dots, c'_{n})$ and $Prop(F)=(f'_{1}, \dots, f'_{m})$.
%Without loss of generality, we identify the components(features) and the variable names $Prop(C)$ ($Prop(F)$). 
If $C$ covers $F$, then $Provided\_by(C)=\{f \mid  \exists C_1 \in prov(f), \exists C_2 \in req(f), C_2 \subseteq C_1 \subseteq C\}$ will contain $F$. 
 Pick $f \in F$.  
Since $\exists C_1 \in prov(f), C_1 \subseteq C$, we have
%Then it can be easily seen that $f \_ implements(c_1, \dots, c_k, f)$ holds for every $f \in F$ since
$\bigwedge_{c \in Prop(C)} c \Rightarrow \bigwedge_{c \in Prop(C_1)} c \Rightarrow formula \_ prov(f)$. 
Therefore, $f \_ implements(c'_{1}, \dots, c'_{n}, f)$ holds ( 
whenever $c'_j=1$, we will have $c_j=1$ in $C$  as well as supersets of $C$; $C$ 
implements $f$ since 
$\bigwedge_{c \in Prop(C)} c \Rightarrow formula \_ prov(f)$) 
 Hence, it will be the case that $f' \Rightarrow f \_ implements(c'_{1}, \dots, c_{n}, f)$ for every 
$f \in F$. Hence, $f \_covers(c'_{1}, \dots, c'_{n}, f'_{1}, \dots, f'_{m})$. 

Conversely, suppose $f \_covers(c'_{1}, \dots, c'_{n}, f'_{1}, \dots, f'_{m})$. 
 Then $\bigwedge_{i=1}^m(f'_i \Rightarrow f \_ implements(c'_{1}, \dots, c'_{n},f_i))$ holds. 
 If  $f \_covers(c'_{1}, \dots, c'_{n}, f'_{1}, \dots, f'_{m})$ holds, then 
(1) either $f'_j=0$, or (2) $f'_j=1$ and $f \_ implements(c'_{1}, \dots, c'_{n},f_j)$ holds. 
As seen in Lemma \ref{impl}, $f \_ implements(c'_{1}, \dots, c'_{n},f_i)$ holds good when there exists a set $C_{j_i} \in prov(f_i)$ such that 
$C_{j_i} \subseteq C$. Since this is true for all $f_i$, we have $\bigcup_{j_i} C_{j_i} \subseteq C$.  
Therefore, $Provided\_by(C) \supseteq Provided\_by(\bigcup_{j_i} C_{j_i})$. By the formula  $f \_covers(c'_{1}, \dots, c'_{n}, f'_{1}, \dots, f'_{m})$, whenever $f'_i=1$, there exists $C_{j_i} \subseteq C$ which implements $f_i$.  
Therefore, $C$ covers $F$.

The proof for realizes is similar. The only difference is that the implication is both ways. 
 
\end{proof}
\begin{lemma}(Completeness, Soundness)
Given an SPL, the SPL is complete iff \\
$\forall f'_1 \dots f'_m[C_F(f'_1, \dots, f'_m) \Rightarrow \exists c'_1 \dots c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_ covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]$

Given an SPL, the SPL is sound iff \\
$\forall c_1 \dots c_n[C_I(c_1, \dots, c_k)] \Rightarrow \exists f_1 \dots f_j[C_F(f_1, \dots, f_j) \wedge f\_ covers(c_1, \dots, c_k, f_1, \dots, f_j)]$
\end{lemma}
\begin{proof}
Assume that the SPL is complete. Then for every $F \in \overline{\cal F}$, there exists some $C \in \overline{\cal C}$ such that $Covers(C,F)$. Pick any $F \in \overline{\cal F}$ and its corresponding $C \in \overline{\cal C}$.
   Let $Prop(F)=(f'_1, \dots, f'_m)$ and $Prop(C)=(c'_1, \dots, c'_n)$. 
Then $C_F(f'_1, \dots, f'_m)$ will be 1 iff there exists a set $S_j \in \overline{\cal F}$ 
such that $Prop(S_j)(i)=1$ iff $f'_i=1$. 
Since $Covers (C,F)$ holds for all $F \in  \overline{\cal F}$, we have by Lemma \ref{rc}, 
$f\_ covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$ is true for every 
tuple $(f'_1, \dots, f'_m)$ such that $f'_i=1$ iff $\exists S_j \in \overline{\cal F}$ 
such that $Prop(S_j)(i)=1$.
 That is, for every tuple $(f'_1, \dots, f'_m)$ that satisfies the feature constraints, 
 there exists some tuple
$(c'_1, \dots, c'_n)$ such that $f\_ covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$ holds. Thus, 
  $\forall f'_1 \dots f'_m.\{[C_F(f'_1, \dots, f'_m) \Rightarrow \exists c'_1 \dots c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]\}$ holds.


Conversely, assume 
$\forall f'_1 \dots f'_m.\{[C_F(f'_1, \dots, f'_m) \Rightarrow \exists c'_1 \dots c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]\}$ holds.
Then for all possible ways of satisfying $C_F(f'_1, \dots, f'_n)$  (i.e, over all $F \in \overline{\cal F}$),
there exists some tuple satisfying $C_I(c'_1, \dots, c'_n)$ such that
$f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$. Each tuple satisfying 
$C_F(f'_1, \dots, f'_n)$ corresponds to a set in $\overline{\cal F}$.
Corresponding to each such set, there is a set 
 $C \in \overline{\cal C}$ with $Prop(C)=(c'_1, \dots, c'_n)$ such that 
$f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$.  This is same as saying that the SPL is complete.

The proof of soundness is similar.
\end{proof}
\begin{lemma}(Existentially Explicit Features)
 Given a set of features $F$, let $Prop(F)=(f'_1, \dots, f'_m)$. Then $F$ is existentially explicit iff 
$\exists c'_1 \dots c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]$. 
\end{lemma}
\begin{proof}
Suppose $F$ is existentially explicit. Then there exists a $C \in \overline{\cal C}$ such that 
$C$ realizes $F$. By Lemma \ref{rc}, $C$ realizes $F$ iff $f\_ realizes(c'_1, \dots, c'_n, f'_1,\dots, f'_m)$.
$C_I(c'_1, \dots, c'_n)$ is true iff there exists a $C \in \overline{\cal C}$ such that 
$Prop(C)=(c'_1, \dots, c'_n)$. Hence, if $F$ is existentially explicit,  
$\exists c'_1, \dots, c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]$ holds.

Conversely, assume \\ 
$\exists c'_1, \dots, c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]$ holds. Then, there exists a $C \in \overline{\cal C}$ with $Prop(C)=(c'_1, \dots, c'_n)$ and 
$f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$. Again, by Lemma \ref{rc}, $f\_realizes(c'_1, \dots, c'_n , f'_1, \dots, f'_m)$ iff $C$ realizes $F$, $Prop(C)=(c'_1, \dots, c'_n), Prop(F)=(f'_1, \dots, f'_m)$. That is, 
for $F \in \overline{\cal F}$, there exists  a $C \in \overline{\cal C}$ such that $C$ covers $F$. Then, 
$F$ is existentially explicit.
 \end{proof}

\begin{lemma}(Universally Explicit Features)
 Given a set of features $F$, let $Prop(F)=(f'_1, \dots, f'_m)$. Then $F$ is universally explicit iff
$\exists c'_1 \dots c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \wedge 
\forall c'_1 \dots c'_n\{[(C_I(c'_1, \dots, c'_n) \wedge f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]
 \Rightarrow f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)\}$.
\end{lemma}
\begin{proof}
Assume $F$ is universally explicit. Then by definition, (i) there exists a $C \in \overline{\cal C}$ such that $C$ realizes $F$ and (ii) for all $C \in \overline{\cal C}$, $C$ covers $F$ $\Rightarrow$ $C$ realizes $F$.

The first point can be expressed as $\exists c'_1 \dots c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]$ - ($C_I(c'_1, \dots, c'_n)$ holds iff there exists a $C \in \overline{\cal C}$ with 
$Prop(C)=(c'_1, \dots, c'_n)$, and $f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$ holds iff $C$ realizes $F$ by Lemma \ref{rc}).
To formalize the second point, we have to consider all possible component tuples $(c'_1, \dots, c'_n)$ satisfying $C_I(c'_1, \dots, c'_n)$, such that $f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$ holds. For each such 
tuple, we have to ensure that $f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$ holds. 
This is true iff 
 $\forall c'_1 \dots c'_n\{[(C_I(c'_1, \dots, c'_n) \wedge f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \Rightarrow f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)\}$ holds.  Clearly, 
if $F$ is universally explicit, then  
$\exists c'_1 \dots c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \wedge 
\forall c'_1 \dots c'_n\{[(C_I(c'_1, \dots, c'_n) \wedge f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \Rightarrow $ \\
$f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)\}$ holds. 

Conversely, assume 
$\exists c'_1 \dots c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \wedge 
\forall c'_1 \dots c'_n\{[(C_I(c'_1, \dots, c'_n) \wedge f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \Rightarrow 
f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)\}$ holds. 
Now, 
$\exists c'_1 \dots c'_n[C_I(c'_1, \dots, c'_n) \wedge f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]$ holds 
whenever there is a tuple $(c'_1, \dots, c'_n)$ satisfying $C_I(c'_1, \dots, c'_n)$ for which 
$f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$ is true. 
This corresponds to a set in $\overline{\cal C}$ with components $Prop(C)=(c'_1, \dots, c'_n)$ which covers $F$. 
 $\forall c'_1 \dots c'_n\{[(C_I(c'_1, \dots, c'_n) \wedge f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \Rightarrow f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)\}$ 
considers all possible tuples $(c'_1, \dots, c'_n)$ satisfying 
$C_I(c'_1, \dots, c'_n) $ for which whenever $f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$ is true, so is 
$f\_realizes(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$. By definition, each tuple satisfying 
$C_I(c'_1, \dots, c'_n) $ corresponds to a set in $\overline{\cal C}$. The formulae holds iff 
for each such $C \in \overline{\cal C}$,  whenever $C$ covers $F$, $C$ realizes $F$. Therefore, $F$ is universally explicit whenever the formula holds.
  
\end{proof}
\begin{lemma}(Unique Implementation)
 Given a set of features $F$, let $Prop(F)=(f'_1, \dots, f'_m)$. Then $F$ has a unique implementation iff 
$\exists c'_1 \dots c'_n[C_I(c'_{1}, \dots, c'_{n}) \wedge f\_covers(c'_{1}, \dots, c'_{n}, f'_1, \dots, f'_m)]
\wedge \forall d'_1 \dots d'_n\{[C_I(d'_{1}, \dots, d'_{n}) \wedge$ \\ $  f\_covers(d'_{1}, \dots, d'_n, f'_1, \dots, f'_m)] \Rightarrow (\wedge_{l=1}^n (d'_i \Leftrightarrow c'_i)\}$
\end{lemma}
\begin{proof}
Let $F$ have a unique implementation. Then there exists a $C \in \overline{\cal C}$ which covers $F$ and 
for all $C' \in \overline{\cal C}$ which covers $F$, $C=C'$. Two architectures $C, C'$ are same 
when $Prop(C)=Prop(C')$. That is,  $Prop(C)(i)=Prop(C')(i)$ for all $1 \leq i \leq n$. 
As given by the definition of $C_I(c'_1, \dots, c'_n)$,  $C_I(c'_1, \dots, c'_n)$ is satisfiable 
iff there exists some  $C \in \overline{\cal C}$ with $Prop(C)=(c'_1, \dots, c'_n)$. 
Such a $C$ covers $F$ iff $f\_covers(c'_{1}, \dots, c'_{n}, f'_1, \dots, f'_m)$ as given by Lemma \ref{rc}. 
We have to check that there is a unique  $C \in \overline{\cal C}$ that can cover $F$ - for this, we enumerate over all possible tuples $(d'_1, \dots, d'_n)$ that satisfy 
$C_I(d'_1, \dots, d'_n)$, and then ensure that $(d'_1, \dots, d'_n)=(c'_1, \dots, c'_n)$.
This is given by 
$\forall d'_1 \dots d'_n\{[C_I(d'_{1}, \dots, d'_{n}) \wedge  f\_covers(d'_{1}, \dots, d'_n, f'_1, \dots, f'_m)] \Rightarrow (\wedge_{l=1}^n (d'_i \Leftrightarrow c'_i)\}$
Thus, if $F$ has a unique implementation, we have 
$\exists c'_1 \dots c'_n[C_I(c'_{1}, \dots, c'_{n}) \wedge f\_covers(c'_{1}, \dots, c'_{n}, f'_1, \dots, f'_m)]
\wedge \forall d'_1 \dots d'_n\{[C_I(d'_{1}, \dots, d'_{n}) \wedge  f\_covers(d'_{1}, \dots, d'_n, f'_1, \dots, f'_m)] \Rightarrow (\wedge_{l=1}^n (d'_i \Leftrightarrow c'_i)\}$ holds.


The converse is similar.

\end{proof}


\begin{lemma}(Common, live and dead elements)
 \begin{enumerate}
  \item A component $c$ is common iff \\
$\forall c'_1, \dots, c'_n, f'_1, \dots, f'_m\{[C_I(c'_{1}, \dots, c'_{n}) \wedge C_F(f'_{1}, \dots, f'_{m})
\wedge f\_covers(c'_{1}, \dots, c'_{n},f'_{1}, \dots, f'_{m})] \Rightarrow c\}$ holds.
\item A component $c$ is live iff \\
$\exists c'_{1}, \dots, c'_{n}, f'_{1}, \dots, f'_{m}\{[C_I(c'_{1}, \dots, c'_{n}) \wedge C_F(f'_{1}, \dots, f'_{m})\wedge f\_covers(c'_{1}, \dots, c'_{n},f'_{1}, \dots, f'_{m}) \wedge c\}$
\item A component $c$ is dead iff \\
$\forall c'_1, \dots, c'_n, f'_1, \dots, f'_m\{[C_I(c'_{1}, \dots, c'_{n}) \wedge C_F(f'_{1}, \dots, f'_{m})
\wedge f\_covers(c'_{1}, \dots, c'_{n},f'_{1}, \dots, f'_{m})] \Rightarrow \neg c\}$ holds.
 \end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}
\item Assume that $c$ is a common component. Then by definition, for all $\langle F, C \rangle \in Prod(\Psi)$,
$c \in C$. To enumerate all possible $\langle F, C \rangle$ for $F \in \overline{\cal F}$ and 
$C \in \overline{\cal C}$, 
 we consider all possible tuples
$(c'_1, \dots, c'_n)$ as well as $(f'_1, \dots, f'_m)$ for which 
$C_I(c'_{1}, \dots, c'_{n}) \wedge C_F(f'_{1}, \dots, f'_{m})$ holds. Clearly, every pair of tuples 
satisfying  $C_I(c'_{1}, \dots, c'_{n}) \wedge C_F(f'_{1}, \dots, f'_{m})$ corresponds 
to a pair $\langle F, C \rangle$. For each such pair $\langle F, C \rangle$ of tuples to be in $Prod(\Psi)$, 
we check if $C$ covers $F$. By Lemma \ref{rc}, this holds iff 
$f\_covers(c'_{1}, \dots, c'_{n},f'_{1}, \dots, f'_{m})$. Clearly, for 
all pairs of tuples for which this is true, if an element is common, then it will 
evaluate to 1. This is given by saying 
$\forall c'_1, \dots, c'_n, f'_1, \dots, f'_m\{[C_I(c'_{1}, \dots, c'_{n}) \wedge C_F(f'_{1}, \dots, f'_{m})
\wedge f\_covers(c'_{1}, \dots, c'_{n},f'_{1}, \dots, f'_{m})] \Rightarrow c\}$. Note that 
$c$ will be 1 in all such tuples iff it is common.
The converse is similar. 

\item Assume $c$ is live. Then there is a pair $\langle F, C \rangle \in Prod(\Psi)$ such that $c \in C$.
The existence of a pair $\langle F, C\rangle \in Prod(\Psi)$ is expressed by saying 
$\exists c'_{1}, \dots, c'_{n},f'_1, \dots, f'_{m}[C_I(c'_{1}, \dots, c'_{n}) \wedge C_F(f'_{1}, \dots, f'_{m})\wedge$ \\ $ f\_covers(c'_{1}, \dots, c'_{n},f'_{1}, \dots, f'_{m})]$. Clearly, if $c$ is in one such tuple, 
it will be 1. This is written by conjuncting $c$ and obtaining 
$\exists c'_{1}, \dots, c'_{n}, f'_{1}, \dots, f'_{m}\{[C_I(c'_{1}, \dots, c'_{n}) \wedge C_F(f'_{1}, \dots, f'_{m})\wedge f\_covers(c'_{1}, \dots, c'_{n},f'_{1}, \dots, f'_{m}) \wedge c\}$. 
The converse is similar.
 
\item This is similar to 1. 
\end{enumerate}

\end{proof}

\begin{lemma}(Superflous)
A component $c_i$ is superflous iff $\forall c'_1, \dots, c'_n,f'_1, \dots,f'_m\{[c'_i \wedge C_I(c'_1, \dots, c'_n) \wedge C_F(f'_1, \dots, f'_m) \wedge f\_covers(c'_1, \dots,c'_i, \dots, c'_n, f'_1, \dots, f'_m)] \Rightarrow \exists d'_1, \dots, d'_n[\neg d'_i \wedge C_I(d'_1, \dots, d'_n) \wedge $ \\ $f\_covers(d'_1, \dots,d'_n, f'_1, \dots, f'_m)]\}$.
\end{lemma}
\begin{proof}
Assume $c_i$ is superflous. Then by definition, for all $C \in \overline{\cal C}$ containing $c_i$ and 
which covers $F$, there exists $C' \in \overline{\cal C}$ which does not contain $c_i$ and which covers $F$, whenever $\langle C, F \rangle \in Prod(\Psi)$.  
First consider all $C \in \overline{\cal C}$ containing $c_i$ which cover $F$. This is given by 
considering all tuples $(c'_1, \dots, c'_n)$ and $(f'_1, \dots, f'_m)$ which satisfy 
$C_I(c'_1, \dots,\dots, c'_n) \wedge C_F(f'_1, \dots, f'_m)$, $c'_i=1$,  and for which 
$f\_covers(c'_1, \dots,c'_i, \dots, c'_n, f'_1, \dots, f'_m)]$ holds (All pairs 
$\langle C, F \rangle$ are enumerated by considering all tuples satisfying 
$C_I(c'_1, \dots, c'_i,\dots, c'_n) \wedge C_F(f'_1, \dots, f'_m)$, and for those in $Prod(\Psi)$, we need to check that $C$ covers $F$. Now, if such a $C$ contains $c_i$, then that $c_i$ is some $c'_i$ in that tuple $(c'_1, \dots, c'_n)$ which is 1). To check if there exists a pair in $Prod(\Psi)$ which does not contain the  $i$th component $c_i$, 
among all tuples $(c'_1, \dots, c'_n)$, we 
check if there exists a tuple $(d'_1, \dots, d'_n)$ such that 
$C_I(d'_1, \dots, d'_n) \wedge f\_covers(d'_1, \dots,d'_n, f'_1, \dots, f'_m)$ holds and 
where $d'_i=0$. This is expressed by $\neg d'_i$. Thus, 
if $c_i$ is superflous, we have 
$\forall c'_1, \dots, c'_n,f'_1, \dots,f'_m\{[c'_i \wedge C_I(c'_1, \dots,  c'_n) \wedge C_F(f'_1, \dots, f'_m) \wedge f\_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \Rightarrow \exists d'_1, \dots, d'_n[\neg d'_i \wedge C_I(d'_1, \dots, d'_n) \wedge f\_covers(d'_1, \dots,d'_n, f'_1, \dots, f'_m)]\}$ holds.

The converse is similar. 
 
\end{proof}

\begin{lemma}(Redundant)
A component $c_i$ is redundant iff $\forall c'_1, \dots, c'_n f'_1 \dots, f'_m\{[c'_i \wedge C_I(c'_1, \dots, c'_n) \wedge C_F(f'_1, \dots, f'_m) \wedge f \_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \Rightarrow \exists d'_1 \dots d'_n[\neg d'_i \wedge (\bigwedge_{i=1}^n c'_i \Rightarrow \bigwedge d'_i) \wedge C_I(d'_1, \dots, d'_n) \wedge $ \\ $
f \_covers(d'_1, \dots, d'_n, f'_1, \dots, f'_m)]\}$.
\end{lemma}
\begin{proof}
Suppose $c_i$ is redundant. Then  for every $C \in \overline{\cal C}$ containing $c_i$, there exists a $C' \in \overline{\cal C}$, $C' \subseteq C$, $c \notin C'$, $Provided \_by(C)=Provided \_by(C')$. First, we have to enumerate all tuples 
$(c'_1, \dots, c'_n)$ for which we have $C_I(c'_1, \dots, c'_n)$ and $c'_i$ (i.e, enumerate all members of $\overline{\cal C}$ containing $c_i$). Now, we have to look at the sets of features $F$ that these architectures cover - by definition of covers, this means that 
the set  $Provided \_ by(C)$ is in $\overline{\cal F}$, and  
 $F \subseteq Provided \_ by(C)$. 
  This basically means to look at all tuples $(f'_1, \dots, f'_m)$ such that 
$C_F(f'_1, \dots, f'_m)$ (which correspond to some element of $\overline{\cal F}$) and
$f \_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)$ (which  are covered by $C$). This is expressed by specifying 
$\forall c'_1, \dots, c'_n, f'_1, \dots, f'_m\{[
 c'_i \wedge C_I(c'_1, \dots, c'_n) \wedge C_F(f'_1, \dots, f'_m) \wedge f \_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)]\}$. For each such $C$ covering $F$, we want to say that there exists  a $C' \subseteq C$ which covers $F$ and which does not contain $c'_i$. This is expressed by saying that there exists a tuple $(d'_1, \dots, d'_n)$ for which 
(i)  $C_I(d'_1, \dots, d'_n)$ holds, (ii) $f \_covers(d'_1, \dots, d'_n, f'_1, \dots, f'_m)$ holds, (iii) $\neg c'_i$ holds, and $(iv)
  (\bigwedge_{i=1}^n c'_i \Rightarrow \bigwedge d'_i)$. This last condition checks that $C' \subseteq C$. Thus, the required formula to hold is 
 $\forall c'_1, \dots, c'_n f'_1 \dots, f'_m\{[c'_i \wedge C_I(c'_1, \dots, c'_n) \wedge C_F(f'_1, \dots, f'_m) \wedge f \_covers(c'_1, \dots, c'_n, f'_1, \dots, f'_m)] \Rightarrow \exists d'_1 \dots d'_n[\neg d'_i \wedge (\bigwedge_{i=1}^n c'_i \Rightarrow \bigwedge d'_i) \wedge C_I(d'_1, \dots, d'_n) \wedge $ \\ $
f \_covers(d'_1, \dots, d'_n, f'_1, \dots, f'_m)]\}$.

The converse is similar.


\end{proof}




\begin{lemma}(Critical)
A component $c$ is critical for $f_j$ iff $\forall c'_1, \dots, c'_n\{[C_I(c'_1, \dots,  c'_n) \wedge f\_implements(c'_1, \dots, c'_n, f_j)] \Rightarrow c\}$. 	
 \end{lemma}
\begin{proof}
Assume $c$ is critical for $f_j$. Then, every architecture which does not contain $c$ 
cannot implement $f_j$. In other words, every architecture in $\overline{\cal C}$ which 
implements  $f_j$ must contain $c$. We enumerate all possible architectures in $\overline{\cal C}$ which implement $f_j$ by considering all tuples $(c'_1, \dots, c'_n)$ for which 
$C_I(c'_1, \dots,  c'_n) \wedge f\_implements(c'_1, \dots, c'_n, f_j)$ holds. If $c$ is in every such architecture, then $c$ will be 1 in all such tuples  
$(c'_1, \dots, c'_n)$. This is checked by saying $c$ holds whenever
$C_I(c'_1, \dots,  c'_n) \wedge f\_implements(c'_1, \dots, c'_n, f_j)$ holds. That is, 
$\forall c'_1, \dots, c'_n\{[C_I(c'_1, \dots,  c'_n) \wedge f\_implements(c'_1, \dots, c'_n, f_j)] \Rightarrow c\}$. 

The converse is similar.

\end{proof}


\begin{lemma}(Extends)
Let $F$ and $F'$ be  subsets of features. Let $Prop(F)=(f_1, \dots, f_m)$ and $Prop(F')=(f'_1, \dots, f'_m)$. Then $F'$ extends $F$ iff $\bigwedge_{i=1}^m (f_i \Rightarrow f'_{i})$ is true. $F'$ is extendable iff $\exists f'_1, \dots, f'_m[\bigwedge_{i=1}^m f_i \Rightarrow f'_{i})]$.
\end{lemma}
\begin{proof}
If $F'$ extends $F$,  then $Prop(F)(i)=1 \Rightarrow Prop(F')(i)=1$. Then clearly, $\bigwedge_{i=1}^m (f_i \Rightarrow f'_{i})$ is true. Conversely, if $\bigwedge_{i=1}^m(f_i \Rightarrow f'_{i})$, then whenever $f_i=1$, $f'_i=1$. That is, $Prop(F)(i)=1 \Rightarrow Prop(F')(i)=1$. Clearly, then $F'$ extends $F$.
If $F$ is extendable, then there exists some $F'$ such that $F'$ extends $F$. This is same as existentially quantifying the variables of $F'$ such that the implication holds.

\end{proof}

